The ANTARES detector: two decades of neutrino searches in the Mediterranean Sea

Interest for studying cosmic neutrinos using deep-sea detectors has increase after the discovery of a diffuse flux of cosmic neutrinos by the IceCube collaboration and the possibility of wider multi-messenger studies with the observations of gravitational waves. The ANTARES detector was the first neutrino telescope in seawater, operating successfully in the Mediterranean Sea for more than a decade and a half. All challenges related to the operation in the deep sea were accurately addressed by the collaboration. Deployment and connection operations became smoother over time; data taking and constant re-calibration of the detector due to the variable environmental conditions were fully automated. A wealth of results on the subject of astroparticle physics, particle physics and multi-messenger astronomy have been obtained, despite the relative modest size of the detector, paving the way to a new generation of larger undersea detectors. This review summarizes the efforts by the ANTARES collaboration that made the possibility to operate neutrino telescopes in seawater a reality and the results obtained in this endeavor.

==> author_list_16032025.tex <==
%\documentclass{elsarticle}
%\journal{}
%\begin{document}
%\begin{frontmatter}
%\title{ANTARES collaboration}
\author[IPHC,UHA]{A.~Albert}
\author[IFIC]{S.~Alves}
\author[UPC]{M.~Andr\'e}
\author[UPV]{M.~Ardid}
\author[UPV]{S.~Ardid}
\author[CPPM]{J.-J.~Aubert}
\author[APC]{J.~Aublin}
\author[APC]{B.~Baret}
\author[LAM]{S.~Basa}
\author[APC]{Y.~Becherini}
\author[CNESTEN]{B.~Belhorma}
\author[Bologna,Bologna-UNI]{F.~Benfenati}
\author[CPPM]{V.~Bertin}
\author[LNS]{S.~Biagi}
\author[Rabat]{J.~Boumaaza}
\author[LPMR]{M.~Bouta}
\author[NIKHEF]{M.C.~Bouwhuis}
\author[ISS]{H.~Br\^{a}nza\c{s}}
\author[NIKHEF,UvA]{R.~Bruijn}
\author[CPPM]{J.~Brunner}
\author[CPPM]{J.~Busto}
\author[Genova]{B.~Caiffi}
\author[IFIC]{D.~Calvo}
\author[Roma,Roma-UNI]{S.~Campion}
\author[Roma,Roma-UNI]{A.~Capone}
\author[Bologna,Bologna-UNI]{F.~Carenini}
\author[CPPM]{J.~Carr}
\author[IFIC]{V.~Carretero}
\author[APC]{T.~Cartraud}
\author[Roma,Roma-UNI]{S.~Celli}
\author[CPPM]{L.~Cerisy}
\author[Marrakech]{M.~Chabab}
\author[Rabat]{R.~Cherkaoui El Moursli}
\author[Bologna]{T.~Chiarusi}
\author[Bari]{M.~Circella}
\author[APC]{J.A.B.~Coelho}
\author[APC]{A.~Coleiro}
\author[LNS]{R.~Coniglione}
\author[CPPM]{P.~Coyle}
\author[APC]{A.~Creusot}
\author[UGR-CITIC]{A.~F.~D\'\i{}az}
\author[CPPM]{B.~De~Martino}
\author[Bologna,Bologna-UNI]{I.~Del~Rosso}
\author[LNS]{C.~Distefano}
\author[Roma,Roma-UNI]{I.~Di~Palma}
\author[APC,UPS]{C.~Donzaud}
\author[CPPM]{D.~Dornic}
\author[IPHC,UHA]{D.~Drouhin}
\author[Erlangen]{T.~Eberl}
\author[Rabat]{A.~Eddymaoui}
\author[NIKHEF]{T.~van~Eeden}
\author[NIKHEF]{D.~van~Eijk}
\author[APC]{S.~El Hedri}
\author[Rabat]{N.~El~Khayati}
\author[CPPM]{A.~Enzenh\"ofer}
\author[Roma,Roma-UNI]{P.~Fermani}
\author[LNS]{G.~Ferrara}
\author[Bologna,Bologna-UNI]{F.~Filippini}
\author[Salerno-UNI]{L.~Fusco}
\author[Roma,Roma-UNI]{S.~Gagliardini}
\author[UPV]{J.~Garc\'\i{}a-Méndez}
\author[NIKHEF]{C.~Gatius~Oliver}
\author[Clermont-Ferrand,APC]{P.~Gay}
\author[Erlangen]{N.~Gei{\ss}elbrecht}
\author[LSIS]{H.~Glotin}
\author[IFIC]{R.~Gozzini}
\author[Erlangen]{R.~Gracia~Ruiz}
\author[Erlangen]{K.~Graf}
\author[Genova,Genova-UNI]{C.~Guidi}
\author[APC]{L.~Haegel}
\author[NIOZ]{H.~van~Haren}
\author[NIKHEF]{A.J.~Heijboer}
\author[GEOAZUR]{Y.~Hello}
\author[Erlangen]{L.~Hennig}
\author[IFIC]{J.J.~Hern\'andez-Rey}
\author[Erlangen]{J.~H\"o{\ss}l}
\author[CPPM]{F.~Huang}
\author[Bologna,Bologna-UNI]{G.~Illuminati}
\author[NIKHEF]{B.~Jisse-Jung}
\author[NIKHEF,Leiden]{M.~de~Jong}
\author[NIKHEF,UvA]{P.~de~Jong}
\author[Wuerzburg]{M.~Kadler}
\author[Erlangen]{O.~Kalekin}
\author[Erlangen]{U.~Katz}
\author[APC]{A.~Kouchner}
\author[Bamberg]{I.~Kreykenbohm}
\author[Genova]{V.~Kulikovskiy}
\author[Erlangen]{R.~Lahmann}
\author[APC]{M.~Lamoureux}
\author[IFIC]{A.~Lazo}
\author[COM]{D.~Lef\`evre}
\author[Catania]{E.~Leonora}
\author[Bologna,Bologna-UNI]{G.~Levi}
\author[CPPM]{S.~Le~Stum}
\author[IRFU/SPP,APC]{S.~Loucatos}
\author[IFIC]{J.~Manczak}
\author[LAM]{M.~Marcelin}
\author[Bologna,Bologna-UNI]{A.~Margiotta}
\author[Napoli,Napoli-UNI]{A.~Marinelli}
\author[UPV]{J.A.~Mart\'inez-Mora}
\author[Napoli]{P.~Migliozzi}
\author[LPMR]{A.~Moussa}
\author[NIKHEF]{R.~Muller}
\author[UGR-CAFPE]{S.~Navas}
\author[LAM]{E.~Nezri}
\author[NIKHEF]{B.~\'O~Fearraigh}
\author[APC]{E.~Oukacha}
\author[ISS]{A.M.~P\u{a}un}
\author[ISS]{G.E.~P\u{a}v\u{a}la\c{s}}
\author[APC]{S.~Pe\~{n}a-Mart\'{\i}nez}
\author[CPPM]{M.~Perrin-Terrin}
\author[LNS]{P.~Piattelli}
\author[Salerno-UNI]{C.~Poir\`e}
\author[ISS]{V.~Popa\fnref{fn1}}
\author[IPHC]{T.~Pradier}
\author[Catania]{N.~Randazzo}
\author[IFIC]{D.~Real}
\author[LNS]{G.~Riccobene}
\author[Genova,Genova-UNI]{A.~Romanov}
\author[IFIC]{A.~S\'anchez~Losa}
\author[IFIC]{A.~Saina}
\author[IFIC]{F.~Salesa~Greus}
\author[NIKHEF,Leiden]{D. F. E.~Samtleben}
\author[Genova,Genova-UNI]{M.~Sanguineti}
\author[LNS]{P.~Sapienza}
\author[IRFU/SPP]{F.~Sch\"ussler}
\author[NIKHEF]{J.~Seneca}
\author[Bologna,Bologna-UNI]{M.~Spurio\corref{cor1}}
\author[IRFU/SPP]{Th.~Stolarczyk}
\author[Genova,Genova-UNI]{M.~Taiuti}
\author[Rabat]{Y.~Tayalati}
\author[IRFU/SPP,APC]{B.~Vallage}
\author[CPPM]{G.~Vannoye}
\author[APC,IUF]{V.~Van~Elewyck}
\author[LNS]{S.~Viola}
\author[Caserta-UNI,Napoli]{D.~Vivolo}
\author[Bamberg]{J.~Wilms}
\author[Genova]{S.~Zavatarelli}
\author[Roma,Roma-UNI]{A.~Zegarelli}
\author[IFIC]{J.D.~Zornoza}
\author[IFIC]{J.~Z\'u\~{n}iga}

\address[IPHC]{\scriptsize{Universit\'e de Strasbourg, CNRS,  IPHC UMR 7178, F-67000 Strasbourg, France}}
\address[UHA]{\scriptsize Universit\'e de Haute Alsace, F-68100 Mulhouse, France}
\address[IFIC]{\scriptsize{IFIC - Instituto de F\'isica Corpuscular (CSIC - Universitat de Val\`encia) c/ Catedr\'atico Jos\'e Beltr\'an, 2 E-46980 Paterna, Valencia, Spain}}
\address[UPC]{\scriptsize{Technical University of Catalonia, Laboratory of Applied Bioacoustics, Rambla Exposici\'o, 08800 Vilanova i la Geltr\'u, Barcelona, Spain}}
\address[UPV]{\scriptsize{Institut d'Investigaci\'o per a la Gesti\'o Integrada de les Zones Costaneres (IGIC) - Universitat Polit\`ecnica de Val\`encia. C/  Paranimf 1, 46730 Gandia, Spain}}
\address[CPPM]{\scriptsize{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}}
\address[APC]{\scriptsize{Universit\'e Paris Cit\'e, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France}}
\address[LAM]{\scriptsize{Aix Marseille Univ, CNRS, CNES, LAM, Marseille, France }}
\address[CNESTEN]{\scriptsize{National Center for Energy Sciences and Nuclear Techniques, B.P.1382, R. P.10001 Rabat, Morocco}}
\address[Bologna]{\scriptsize{INFN - Sezione di Bologna, Viale Berti-Pichat 6/2, 40127 Bologna, Italy}}
\address[Bologna-UNI]{\scriptsize{Dipartimento di Fisica e Astronomia dell'Universit\`a di Bologna, Viale Berti-Pichat 6/2, 40127, Bologna, Italy}}
\address[LNS]{\scriptsize{INFN - Laboratori Nazionali del Sud (LNS), Via S. Sofia 62, 95123 Catania, Italy}}
\address[Rabat]{\scriptsize{University Mohammed V in Rabat, Faculty of Sciences, 4 av. Ibn Battouta, B.P. 1014, R.P. 10000 Rabat, Morocco}}
\address[LPMR]{\scriptsize{University Mohammed I, Laboratory of Physics of Matter and Radiations, B.P.717, Oujda 6000, Morocco}}
\address[NIKHEF]{\scriptsize{Nikhef, Science Park,  Amsterdam, The Netherlands}}
\address[ISS]{\scriptsize{Institute of Space Science - INFLPR subsidiary, 409 Atomistilor Street, M\u{a}gurele, Ilfov, 077125 Romania}}
\address[UvA]{\scriptsize{Universiteit van Amsterdam, Instituut voor Hoge-Energie Fysica, Science Park 105, 1098 XG Amsterdam, The Netherlands}}
\address[Genova]{\scriptsize{INFN - Sezione di Genova, Via Dodecaneso 33, 16146 Genova, Italy}}
\address[Roma]{\scriptsize{INFN - Sezione di Roma, P.le Aldo Moro 2, 00185 Roma, Italy}}
\address[Roma-UNI]{\scriptsize{Dipartimento di Fisica dell'Universit\`a La Sapienza, P.le Aldo Moro 2, 00185 Roma, Italy}}
\address[Marrakech]{\scriptsize{LPHEA, Faculty of Science - Semlali, Cadi Ayyad University, P.O.B. 2390, Marrakech, Morocco.}}
\address[Bari]{\scriptsize{INFN - Sezione di Bari, Via E. Orabona 4, 70126 Bari, Italy}}
\address[UGR-CITIC]{\scriptsize{Department of Computer Architecture and Technology/CITIC, University of Granada, 18071 Granada, Spain}}
\address[UPS]{\scriptsize{Universit\'e Paris-Sud, 91405 Orsay Cedex, France}}
\address[Erlangen]{\scriptsize{Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, Erwin-Rommel-Str. 1, 91058 Erlangen, Germany}}
\address[Salerno-UNI]{\scriptsize{Universit\`a di Salerno e INFN Gruppo Collegato di Salerno, Dipartimento di Fisica, Via Giovanni Paolo II 132, Fisciano, 84084 Italy}}
\address[Clermont-Ferrand]{\scriptsize{Laboratoire de Physique Corpusculaire, Clermont Universit\'e, Universit\'e Blaise Pascal, CNRS/IN2P3, BP 10448, F-63000 Clermont-Ferrand, France}}
\address[LSIS]{\scriptsize{LIS, UMR Universit\'e de Toulon, Aix Marseille Universit\'e, CNRS, 83041 Toulon, France}}
\address[Genova-UNI]{\scriptsize{Dipartimento di Fisica dell'Universit\`a, Via Dodecaneso 33, 16146 Genova, Italy}}
\address[NIOZ]{\scriptsize{Royal Netherlands Institute for Sea Research (NIOZ), Landsdiep 4, 1797 SZ 't Horntje (Texel), the Netherlands}}
\address[GEOAZUR]{\scriptsize{G\'eoazur, UCA, CNRS, IRD, Observatoire de la C\^ote d'Azur, Sophia Antipolis, France}}
\address[Leiden]{\scriptsize{Huygens-Kamerlingh Onnes Laboratorium, Universiteit Leiden, The Netherlands}}
\address[Wuerzburg]{\scriptsize{Institut f\"ur Theoretische Physik und Astrophysik, Universit\"at W\"urzburg, Emil-Fischer Str. 31, 97074 W\"urzburg, Germany}}
\address[Bamberg]{\scriptsize{Dr. Remeis-Sternwarte and ECAP, Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg,  Sternwartstr. 7, 96049 Bamberg, Germany}}
\address[COM]{\scriptsize{Mediterranean Institute of Oceanography (MIO), Aix-Marseille University, 13288, Marseille, Cedex 9, France; Universit\'e du Sud Toulon-Var,  CNRS-INSU/IRD UM 110, 83957, La Garde Cedex, France}}
\address[Catania]{\scriptsize{INFN - Sezione di Catania, Via S. Sofia 64, 95123 Catania, Italy}}
\address[IRFU/SPP]{\scriptsize{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}}
\address[Napoli]{\scriptsize{INFN - Sezione di Napoli, Via Cintia 80126 Napoli, Italy}}
\address[Napoli-UNI]{\scriptsize{Dipartimento di Fisica dell'Universit\`a Federico II di Napoli, Via Cintia 80126, Napoli, Italy}}
\address[UGR-CAFPE]{\scriptsize{Dpto. de F\'\i{}sica Te\'orica y del Cosmos \& C.A.F.P.E., University of Granada, 18071 Granada, Spain}}
\address[IUF]{\scriptsize{Institut Universitaire de France, 75005 Paris, France}}
\address[Caserta-UNI]{\scriptsize{Dipartimento di Matematica e Fisica dell'Universit\`a della Campania L. Vanvitelli, Via A. Lincoln, 81100, Caserta, Italy}}
%
\cortext[cor1]{Corresponding author: maurizio.spurio@unibo.it}
\fntext[fn1]{Deceased}
%\end{frontmatter}
%\end{document}

